Differentially Private Projected Histograms of Multi-Attribute Data for Classification

In this paper, we tackle the problem of constructing a differentially private synopsis for the classification analyses. Several the state-of-the-art methods follow the structure of existing classification algorithms and are all iterative, which is suboptimal due to the locally optimal choices and the over-divided privacy budget among many sequentially composed steps. Instead, we propose a new approach, PrivPfC, a new differentially private method for releasing data for classification. The key idea is to privately select an optimal partition of the underlying dataset using the given privacy budget in one step. Given one dataset and the privacy budget, PrivPfC constructs a pool of candidate grids where the number of cells of each grid is under a data-aware and privacy-budget-aware threshold. After that, PrivPfC selects an optimal grid via the exponential mechanism by using a novel quality function which minimizes the expected number of misclassified records on which a histogram classifier is constructed using the published grid. Finally, PrivPfC injects noise into each cell of the selected grid and releases the noisy grid as the private synopsis of the data. If the size of the candidate grid pool is larger than the processing capability threshold set by the data curator, we add a step in the beginning of PrivPfC to prune the set of attributes privately. We introduce a modified $\chi^2$ quality function with low sensitivity and use it to evaluate an attribute's relevance to the classification label variable. Through extensive experiments on real datasets, we demonstrate PrivPfC's superiority over the state-of-the-art methods.

==> preliminaries.tex <==
\subsection{Differential Privacy} \label{sec:preliminaries:differential}

Informally, differential privacy requires that the output of a data analysis mechanism be approximately the same, even if any single tuple in the input database is arbitrarily added or removed.
\begin{definition}[{$\epsilon$-Differential Privacy~\cite{Dwo06,DMNS06}}] \label{def:diff}
A randomized mechanism $\AA$ gives $\epsilon$-differential privacy if for any pair of neighboring datasets $D$ and $D'$, and any $S\in \mathit{Range}(\AA)$,
%\begin{equation}\label{eqn:dp}
$$\Pr{\AA(D)=S} \leq e^{\epsilon}\cdot \Pr{\AA(D')=S}.$$
%\end{equation}
\end{definition}

In this paper we consider two datasets $D$ and $D^{\prime}$ to be neighbors if and only if either $D=D' + t$ or $D'=D + t$, where $D +t$ denotes the dataset resulted from adding the tuple $t$ to the dataset $D$. We use $D\simeq D'$ to denote this.  This protects the privacy of any single tuple, because adding or removing any single tuple results in $e^{\epsilon}$-multiplicative-bounded changes in the probability distribution of the output.
%If any adversary can make certain inference about a tuple based on the output, then the same inference is also likely to occur even if the tuple does not appear in the dataset.

%An alternative is to define $D$ and $D'$ to be neighbors when they contain the same number of tuples and all except for one are the same.  When the number of tuples in the input dataset is not sensitive, either of these two notions offers sufficient privacy protection.


%Jianneng: if later we need to apply exponential mechanism, we use the following paragraph
%There are several approaches for designing  mechanisms that satisfy $\epsilon$-differential privacy.  In this paper we use two of them.  The first approach computes a function $g$ on the dataset $D$ in a differentially privately way, by adding to $g(D)$ a random noise.  The magnitude of the noise depends on $\mathsf{GS}_f$, the \emph{global sensitivity} or the $L_1$ sensitivity of $g$.  Such a mechanism $\AA_g$ is given below:


\begin{comment}
There are several approaches for designing mechanisms that satisfy $\epsilon$-differential privacy, including Laplace mechanism \cite{DMNS06}, Exponential mechanism \cite{MT07}, and Geometric mechanism \cite{GRS09}. In this paper we use Laplace mechanism.  It computes a function $g$ on the dataset $D$ in a differentially privately way, by adding to $g(D)$ a random noise.  The magnitude of the noise depends on $\mathsf{GS}_g$, the \emph{global sensitivity} or the $L_1$ sensitivity of $g$.  Such a mechanism $\AA_g$ is given below:
$$
\begin{array}{crl}
& \AA_g(D) & =g(D)+\mathsf{Lap}\left(\frac{\mathsf{GS}_g}{\epsilon}\right)
  \\
\mbox{where} &  \mathsf{GS}_g & = \max\limits_{(D,D') : D \simeq D'} |g(D) - g(D')|,
\\
\mbox{and}& \Pr{\Lap{\beta}=x} & = \frac{1}{2\beta} \myexp{-|x|/\beta}
\end{array}
$$
In the above, $\Lap{\beta}$ denotes a random variable sampled from the Laplace distribution with scale parameter $\beta$. %This is generally referred to as the \emph{Laplacian mechanism} for satisfying differential privacy.
\end{comment}


There are several primitives for satisfying $\epsilon$-differential privacy.  In this paper we use two of them.  The first primitive is to add a random noise sampled from a distribution with the scale parameter proportional to $\mathsf{GS}_f$, the \emph{global sensitivity} or the $L_1$ sensitivity of the function $f$.  That is, we use $\AA_f$ to compute $f$ on a dataset $D$, where:
$$
\begin{array}{crl}
& \AA_f(D) & =f(D)+\mathsf{Lap}\left(\frac{\mathsf{GS}_f}{\epsilon}\right),\\
\mbox{where} &  \mathsf{GS}_f & = \max_{D\simeq D'} |f(D) - f(D')|,
\\
\mbox{and}& \Pr{\Lap{\beta}=x} & = \frac{1}{2\beta} \myexp{-|x|/\beta}.
\end{array}
$$
In the above, $\Lap{\beta}$ denotes a random variable sampled from the Laplace distribution with scale parameter $\beta$. This is generally referred to as the \emph{Laplacian mechanism}~\cite{DMNS06} for satisfying differential privacy.

Another primitive is to sample the output of the data analysis mechanism according to an exponential distribution; this is generally referred to as the \emph{exponential mechanism}~\cite{MT07}.  The mechanism relies on a \emph{quality} function $q: \mathcal{D} \times \mathcal{R} \rightarrow \mathbb{R}$ that assigns a real valued score to one output $r\in\mathcal{R}$ when the input dataset is $D$, where higher scores indicate more desirable outputs.  Given the quality function $q$, its global sensitivity $\mathsf{GS}_q$ is defined as:
\begin{equation*}
\mathsf{GS}_q = \max_{r} \max_{D\simeq D'} |q(D,r) - q(D',r)|.
\end{equation*}

The following method satisfies $\epsilon$-differential privacy:
\begin{equation*}
 \Pr{r\mbox{ is selected}} \propto \myexp{\left(\frac{\epsilon }{2\,\mathsf{GS}_q}q(D,r)\right)}.  \label{eq:exp}
\end{equation*}

Differential privacy is sequentially composable in the sense that combining multiple mechanisms $\AA_{1}, \cdots, \AA_{m}$ that satisfy differential privacy for $\epsilon_1, \cdots,\epsilon_m$ results in a mechanism that satisfies $\epsilon$-differential privacy for $\epsilon=\sum_{i} \epsilon_i$.  %Because of this, we refer to $\epsilon$ as the privacy budget of a privacy-preserving data analysis task.
When a task involves multiple steps, each step uses a portion of $\epsilon$ so that the sum of these portions is no more than $\epsilon$.  
%Differential privacy is also parallelly composable.  Suppose the data is partitioned into $m$ arbitrary disjoint subsets and mechanism $\AA_{i}$ is executed on the $i$'th subset.  The parallel execution of $\AA_{1}, \cdots, \AA_{m}$ satisfies $\max_{i}(\epsilon_{i})$-differential privacy.




\begin{comment}
\subsection{Classification}\label{sec:preliminaries:histogram-classifier}
In machine learning, classification is the problem of predicting the unknown category label of a new observation, based on a training set of data which contains observations whose category label is known.  And the goal of classification is to determine a mapping or a classifier, $f:\mathcal{X} \rightarrow \mathcal{Y}$ that takes an input $x\in\mathcal{X}$ and predicts the corresponding output $y\in\mathcal{Y}$.  Given one test tuple $\{X, Y\}\in \{\mathcal{X}, \mathcal{Y}\}$, the performance of a classifier $f$ is measured by its expected loss,
\begin{equation*}
R(f) = \mathrm{E}_{XY}[l(f(X), Y)],% =\Pr_{XY}[f(X) \neq Y]
\end{equation*}
where $l(f(X), Y)$ is the 0/1 loss function,
\begin{align*}
	l(f(x), y) =
	\begin{dcases}
		1,  & \text{if } f(x) \neq y,\\
		0, & \text{otherwise}.
	\end{dcases}
\end{align*}
The quality of a classifier can also be viewed as the misclassification rate, the ratio of the number of incorrect classifications to the total number of classifications.
%However, the risk $R(f)$ cannot be computed because the full distribution of $X$ and $Y$ is unknown to the learning algorithm.  People can compute an alternative, empirical risk, by averaging the loss function over the training dataset


\begin{equation}
\hat{R}_{n}(f) = \frac{1}{n}\sum_{i=1}^{n} l(f(X_{i}), Y_{i}).
\end{equation}
And empirical risk minimization is the process of choosing a mapping which minimizes the empirical risk
\begin{equation}
\hat{f}_{n} = \argmin_{f\in\mathcal{F}} \hat{R}_{n}(f).
\end{equation}
To avoid the overfitting in the empirical risk minimization, one common approach is complexity penalization method which add an extra cost associated to the model. Ahe the above process becomes
\begin{equation}
\hat{f}_{n} = \argmin_{f\in\mathcal{F}} \{\hat{R}_{n}(f) + C(f)\},
\end{equation}
where $C(f)$ reflects the complexity of the model.

Example of classification algorithms include decision trees and support vector machines (SVM).

There is a best possible classifier, $f^{*}$, called Bayes classifier, such that
\begin{equation}
f^{*} = \argmin_{f: \mathcal{X} \rightarrow \mathcal{Y}} R(f).
\end{equation}
The Bayes classifier is the following mapping
\begin{definition}[Bayes Classifier]\label{bayesclassifier}
\begin{align}\label{eq:eta}
	h^{*}(x) =
	\begin{dcases}
		1,  & \text{if } \eta(x) = \Pr{Y = 1|X = x} \geq 1/2\\
		0, & \text{otherwise}
	\end{dcases}
\end{align}
\end{definition}
Given the training data, one way to construct a classifier is to estimate the $\eta(\cdot)$ function and plug it in the form of Bayes classifier.  To construct the Bayes classifier, one needs to estimate $\eta$.  And one way to estimate $\eta(\cdot)$ is to partition the data space and therefore approximate the data distribution.  In this approach, the data space can be partitioned uniformly or nonuniformly.



\end{comment}


%Another way is to find a linear plane which can separate the points with different class label as much as possible.  In this paper, we focus on the partitioning approach.


\begin{comment}
The construction of the classifier is also the process to approximate the data distribution.   There are multiple ways to construct classifiers, such as the support vector machine or the decision tree.  However, there also exists a much simpler approach, which uniformly partitions the whole data space into equal size cells and performs majority voting in each cell to determine its class label. This approach is called \emph{histogram classifier}~\cite{DGL96, Nowak09}.

\begin{definition}[Histogram Classifier]\label{histclassifier}
The histogram classifier is based on partitioning the data space $\mathcal{X}$ into $M$ disjoint cells $Q_{1}, Q_{2},\ldots, Q_{M}$.  Given the training data $\{X_i, Y_i\}_{i=1}^{n}$, do cell counting and majority voting to decide the class label of each cell.  Given one test tuple $\{X, Y\}$, the histogram classifiers use the label of the cell where $X$ belongs as the prediction of $Y$.  Specially,
\begin{align*}
	f(X) =
	\begin{dcases}
		1,  &\text{if } \sum_{i=1}^{n}\mathbf{I}_{\{Y_{i} = 1\}}\mathbf{I}_{\{X_{i}\in Q(X)\}} \geq \sum_{i=1}^{n}\mathbf{I}_{\{Y_{i} = 0\}}    \mathbf{I}_{\{X_{i}\in Q(X)\}}\\
		0, &\text{otherwise},
	\end{dcases}
\end{align*}
where $Q(X)$ denotes the cell containing $X$.
\end{definition}
\end{comment}

\begin{comment}
Suppose we have $d$ numerical features and all of them are randomly distributed over the unit hypercube $\chi = [0, 1]^d$.  And assume that we have two classes, $\{0,1\}$.
\begin{definition}[Histogram Classifier]\label{histclassifier}
The histogram classifier is based on partitioning the hypercube $[0,1]^d$ into $M$ cells of equal size, $\{Q_i\}, i = 1, \ldots, M$.  Given the training data $\{X_i, Y_i\}_{i=1}^{n}$, do cell counting and majority voting to decide the class label of each cell.  Given one test data $\{X, Y\}$, the histogram classifiers use the label of the cell where $X$ belongs as the prediction of $Y$.  Specially, the following $\hat{\eta}_{n}(x)$ is an approximation of the $\eta(x)$ in the definition of the Bayes classifier.

\begin{equation}\label{etaapprox}
\hat{\eta}_{n}(x) = \sum_{j = 1}^{M} \hat{P}_j \mathbf{1}\{x\in Q_j\},
\end{equation}
where
\begin{align*}
	\hat{P}_j =
	\begin{dcases}
		\frac{\sum_{i=1}^{n}\mathbf{1}\{X_{i}\in Q_j, Y_i = 1\}}{\sum_{i=1}^{n}\mathbf{1}\{X_{i}\in Q_j\}},  & \text{if } \sum_{i=1}^{n}\mathbf{1}\{X_{i}\in Q_j\} \neq 0\\
		0, & \text{otherwise}.
	\end{dcases}
\end{align*}
\end{definition}
\end{comment}


\begin{comment}
The regularized empirical risk of the histogram classifier is
\begin{equation}
\min_{f\in\mathcal{F}} \hat{R}_{n}(f) + \sqrt{\frac{2k\log(2) + \frac{1}{2}\log(n)}{2n}}.
\end{equation}


An example of non-uniform partition is the decision tree classifier.  The tree construction is based on recursively partition the data space over selected dimensions.  And the tree divides the data space into axis-parallel rectangles, each labels with the majority class.  Compared with the above histogram classifier, the decision tree classifier locates the decision tree boundary better.
\end{comment}



\begin{comment}
Even the "perfect" bayes classifier cannot achieve zero error. This is because the data distribution cannot always be separated into two non-overlapping parts. Those overlapping parts cannot be classified since the points inside has contradictory class labels and therefore constitute the irreducible part in the classification error.

It can be proved that the Bayes classifier can achieve the minimum expected risk of all classifiers.
\begin{equation}
R(f^{*}) = \inf_{f} R(f).
\end{equation}
\end{comment}

%Jianneng: so far we do not use exponential mechanism.
\begin{comment}
The second approach computes a function $g$ on a dataset $D$ by sampling from the set of all possible answers in the range of $g$ according to an exponential distribution, with answers that are ``more accurate'' will be sampled with higher probability.  This is generally referred to as the \emph{exponential mechanism}~\cite{MT07}.
This approach requires the specification of a \emph{quality} function $q: \mathcal{D} \times \mathcal{R} \rightarrow \mathbb{R}$, where the real valued score $q(D,r)$ indicates how accurate it is to return $r$ when the input dataset is $D$.  Higher scores indicate more accurate outputs which should be returned with higher probabilities. Given the quality function $q$, its global sensitivity $\mathsf{GS}_q$ is defined as:
$$ \mathsf{GS}_q = \max_{r} \max_{(D,D'):D\simeq D'} |q(D,r) - q(D',r)| $$
The following method $\MM$ satisfies $\epsilon$-differential privacy:
\begin{equation}
 \Pr{\MM(D)=r} \propto \exp{\left(\frac{\epsilon }{2\,\mathsf{GS}_q}q(D,r)\right)} \label{eq:exp}
\end{equation}
For example, if $q(D,r_1)-q(D,r_2)=1$, then $r_1$ should be returns $y$ times more likely than $r_2$, with
$y=\exp{\left(\frac{\epsilon }{2\,\mathsf{GS}_q}\right)}$.  The larger the exponent $\frac{\epsilon }{2\,\mathsf{GS}_q}$ is, the more likely that \MM will return the higher quality result.

As pointed out in~\cite{MT07}, in some cases the quality function satisfies the condition that when the input dataset is changed from $D$ to $D'$, the quality values of all outcomes change only in one direction, i.e.,
$$\forall_{D\simeq D'}
\!\left[\left(\exists_{r_1}\, q(D,r_1) \!<\! q(D',r_1)\right) \!\rightarrow\! \left(\forall_{r_2}\,q(D,r_2) \!\leq \! q(D',r_2)\right)\right]$$
Then one can remove the factor of $1/2$ in the exponent of Equation~(\ref{eq:exp}) and return $r$ with probability proportional to $\exp\!{\left(\frac{\epsilon }{\mathsf{GS}_q}q(D,r)\right)}$.  This improves the accuracy of the result.
\end{comment}
\begin{comment}
the following mechanism satisfies $\epsilon$-differential privacy:
	$$\Pr{\MM(D)=r} \propto \exp{\left(\frac{\epsilon q(D,r)}{\mathsf{GS}_q}\right)}.$$
This method samples an output $r$ proportional to $\exp{\left(\epsilon q(D,r)/ \mathsf{GS}_q\right)}$.
\end{comment}












